P2L: Predicting Transfer Learning for Images and Semantic Relations

Transfer learning enhances learning across tasks, by leveraging previously learned representations -- if they are properly chosen. We describe an efficient method to accurately estimate the appropriateness of a previously trained model for use in a new learning task. We use this measure, which we call "Predict To Learn" ("P2L"), in the two very different domains of images and semantic relations, where it predicts, from a set of "source" models, the one model most likely to produce effective transfer for training a given "target" model. We validate our approach thoroughly, by assembling a collection of candidate source models, then fine-tuning each candidate to perform each of a collection of target tasks, and finally measuring how well transfer has been enhanced. Across 95 tasks within multiple domains (images classification and semantic relations), the P2L approach was able to select the best transfer learning model on average, while the heuristic of choosing model trained with the largest data set selected the best model in only 55 cases. These results suggest that P2L captures important information in common between source and target tasks, and that this shared informational structure contributes to successful transfer learning more than simple data size.

==> ccdbp-experiments.tex <==
%First we show performance of each of the source models on the source task, as well as basic statistics about each task.

Figure \ref{fig.ccdbpBinaryCS} shows the correlation of the prediction $E(t_i,s_j)$ with the improvement $I(t_i,s_j)$, when using KLD in addition to size of the source domains' training set in $E$. Figure \ref{fig.ccdbpBinaryS} shows the same when only size is used.  Using the estimator produced better predictions, that is, $E(t_i,s_j)$ and $I(t_i,s_j)$ were then better correlated (Spearman's $\rho$ = .747, Pearson's $R$ = .847).

\begin{figure}[htb]
   \centering
	\begin{minipage}{.5\textwidth}
	\centering
   \includegraphics[width=.9\linewidth]{figures/ccdbpBinaryNF.pdf}
   \caption{Transfer Learning Improvement\\ Predicted by KLD with Size for CCDBP}
   \label{fig.ccdbpBinaryCS}
	\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
   \includegraphics[width=.9\linewidth]{figures/ccdbpBinaryS2short.pdf}
   \caption{Transfer Learning Improvement\\ Predicted by Size for CCDBP}
   \label{fig.ccdbpBinaryS}
	\end{minipage}
\end{figure}


%Figure \ref{fig.ccdbpBinaryC} shows the correlation of the prediction $E(t_i,s_j)$ with the improvement $I(t_i,s_j)$ when only the distance measure is used for $E$. Figure \ref{fig.ccdbpBinaryS} shows the same when only the size of the source domain's training set is used for $E$. Finally, the combination of the distance measure with the training set size gives Figure \ref{fig.ccdbpBinaryCS}, showing the highest correlation between $E(t_i,s_j)$ and $I(t_i,s_j)$.

%\begin{figure}[htb]
%   \centering
%	\begin{minipage}{.5\textwidth}
%	\centering
%   \includegraphics[width=.9\linewidth]{figures/ccdbpBinaryC.pdf}
%   \caption{Transfer Learning Improvement\\ Predicted by KLC}
%   \label{fig.ccdbpBinaryC}
%	\end{minipage}%
%\begin{minipage}{.5\textwidth}
%  \centering
%   \includegraphics[width=.9\linewidth]{figures/ccdbpBinaryS.pdf}
%   \caption{Transfer Learning Improvement\\ Predicted by Size}
%   \label{fig.ccdbpBinaryS}
%	\end{minipage}
%\end{figure}

%\begin{figure*}[htb]
%   \centering
%		\begin{minipage}{.5\textwidth}
%		\centering
%   \includegraphics[width=.9\textwidth]{figures/ccdbpBinaryCS.pdf}
%   \caption{Transfer Learning Improvement\\ Predicted by KLC with Size}
%   \label{fig.ccdbpBinaryCS}
%	\end{minipage}%
%\begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.9\textwidth]{figures/ensembleResults.pdf}
%   \caption{Ensembling top vs. bottom predictions}
%   \label{fig.ccdbpEnsemble}
%	\end{minipage}
%\end{figure*}




%Bhatta : commenting to save space : We are concerned with the case where attempting transfer learning from all source models is unreasonably expensive. But we may have the computational resources to train multiple models transferred from different sources. In this case we can construct an ensemble. To compute the prediction of the ensemble we use the simple strategy of simply averaging the scores of the models.

%Bhatta: commenting to save space : For each of the seven target domains, there are six different source models we may transfer from. We compare an ensemble of the three models predicted to have the worst performance to an ensemble of the three models predicted to have the best performance.

%hatta: commenting to save space : Figure \ref{fig.ccdbpEnsemble} shows the results. In most cases, ensembling all models results in the best performance. But given the constraint where only three models may be selected to train, using the three top predictions far outperforms using the three bottom predictions. 

%\begin{tabular}{r|r|r|r|r}
%Division Name & Best Single Model & Full Ensemble & Bottom Predictions & Top Predictions \\
%\hline
%coparticipatesWith & 0.6648 & 0.7039 & 0.6305 & 0.7161\\
%hasLocation & 0.7572 & 0.7906 & 0.7488 & 0.7822\\
%sameSettingAs & 0.6347 & 0.6488 & 0.5865 & 0.6597 \\
%isClassifiedBy & 0.7472 & 0.8065 & 0.7712 & 0.7909 \\
%hasPart & 0.7057 & 0.7574 & 0.7040 & 0.7396 \\
%hasMember & 0.8549 & 0.8682 & 0.8067 & 0.8795 \\
%hasRole & 0.8278 & 0.8728 & 0.8203 & 0.8676 \\
%\end{tabular}
%TODO: compare voting ensemble of three (predicted) best vs. three (predicted) worst

%Target = 6
%Source 0: AUC = 0.7858457210906692
%Source 1: AUC = 0.8163250070619567
%Source 2: AUC = 0.7806702981028328
%Source 3: AUC = 0.8115366742918494
%Source 4: AUC = 0.7070769401650284
%Source 5: AUC = 0.8277506993869063
%Voting: AUC = 0.872815357982227
%Vote 3 worst: AUC = 0.8202645821440903
%Vote 3 best: AUC = 0.8675818884368459

%Target = 0
%Source 1: AUC = 0.6648432700583397
%Source 2: AUC = 0.6370708527939907
%Source 3: AUC = 0.5782054427688702
%Source 4: AUC = 0.5597265818487781
%Source 5: AUC = 0.6133265251283397
%Source 6: AUC = 0.5277562097435273
%Voting: AUC = 0.7039126414567123
%Vote 3 worst: AUC = 0.6304896423032798
%Vote 3 best: AUC = 0.7160641193855322
%Target = 1
%Source 0: AUC = 0.7572211590525328
%Source 2: AUC = 0.7025035071851392
%Source 3: AUC = 0.692967903318755
%Source 4: AUC = 0.707878066970348
%Source 5: AUC = 0.6873762857193991
%Source 6: AUC = 0.6496294816749236
%Voting: AUC = 0.7906277746340198
%Vote 3 worst: AUC = 0.7487629155673763
%Vote 3 best: AUC = 0.7822050175098472
%Target = 2
%Source 0: AUC = 0.6346921992631886
%Source 1: AUC = 0.5868588537038666
%Source 3: AUC = 0.5421126384609848
%Source 4: AUC = 0.48839832362490787
%Source 5: AUC = 0.5389696014930436
%Source 6: AUC = 0.4823904808271149
%Voting: AUC = 0.648769374568575
%Vote 3 worst: AUC = 0.5864649896013729
%Vote 3 best: AUC = 0.6597027504148946
%Target = 3
%Source 0: AUC = 0.7472087613338148
%Source 1: AUC = 0.7402043751696549
%Source 2: AUC = 0.6827409451713298
%Source 4: AUC = 0.6696407806276876
%Source 5: AUC = 0.6946154282654166
%Source 6: AUC = 0.6349101275807342
%Voting: AUC = 0.8065393485798867
%Vote 3 worst: AUC = 0.7712075765926609
%Vote 3 best: AUC = 0.7909402743444376
%Target = 4
%Source 0: AUC = 0.6222731523907583
%Source 1: AUC = 0.7057050992871291
%Source 2: AUC = 0.6522014197485306
%Source 3: AUC = 0.6321462230107009
%Source 5: AUC = 0.6129898482918226
%Source 6: AUC = 0.5958084286810433
%Voting: AUC = 0.7574251406157161
%Vote 3 worst: AUC = 0.703998969258845
%Vote 3 best: AUC = 0.7396209523667557
%Target = 5
%Source 0: AUC = 0.8277618726144577
%Source 1: AUC = 0.85491750371724
%Source 2: AUC = 0.8047798606586042
%Source 3: AUC = 0.7452124788690435
%Source 4: AUC = 0.7170796796157723
%Source 6: AUC = 0.7491547624359142
%Voting: AUC = 0.8682148208401013
%Vote 3 worst: AUC = 0.8066634366075967
%Vote 3 best: AUC = 0.8795410545179846


%TODO: table of correlation coefficients per distance metric

%training target models with and without transfer learning

%show transfer results

%CONSIDER: show performance of source models relative to training on entire dataset (how much multitask matters)

%train/test of source models


%In addition to the binary relation types, we consider the recently introduced unary approach to relation extraction \cite{unaryRelations}.
%These divisions are shown in Table \ref{tbl.ccdbpSourceUnary}.
%
%\begin{figure}
%\begin{tabular}{r|r|r}
%Division Name & Number of Relations & Positives in Train \\
%\hline
%hasLocation	& 119 & 301646 \\
%isClassifiedBy	& 96 & 162854 \\
%birthYear	& 96 & 152612 \\
%genre/occupation	& 96 & 154669 \\
%activeYearsStart/hasRole	& 96 & 165564 \\
%participatesWith/type/recordLabel	& 96 & 124438 \\
%birthPlace/sameSettingAs/activeYearsEnd	& 96 & 150742 \\
%releaseYear/country/timeZone	& 95 & 211783 \\
%\end{tabular}
%\caption{Source domains division of CC-DBP for unary relation extraction}
%\label{tbl.ccdbpSourceUnary}
%\end{figure}



==> ccdbp.tex <==
\newcommand{\kbent}[1]{\textsc{#1}}
\newcommand{\kbrel}[1]{\textit{#1}}
\newcommand{\kbtrip}[3]{$\langle \kbent{#1}\ \kbrel{#2}\ \kbent{#3} \rangle$}

%Explain the task.
%What is KBP? What is DBpedia? How do you prediction relations from textual evidence? Is this the same as information extraction? What's mention level vs. knowledge level?


The task of relation prediction provides a second benchmark for source domain selection.  
In this task, a knowledge base is extended with information extracted from text. 
We use the CC-DBP~\cite{ccdbp} dataset: the text of Common Crawl\footnote{\url{http://commoncrawl.org}} and the knowledge schema and training data from DBpedia~\cite{dbpedia}.

%DBpedia is a knowledge graph extracted from the infoboxes from Wikipedia. %The fields of the infoboxes are mapped into a knowledge schema. This schema also has a hierarchy of relations, grouping basic relations into more abstract, high level relations.
%A simple example is the \kbrel{hasMember}~/ \kbrel{isMemberOf} relation, which groups relations such as \kbrel{employer}, \kbrel{bandMember} and (political) \kbrel{party}. 

%Examples of each relation. Both a triple and in text.

DBpedia is a knowledge graph extracted from the infoboxes from Wikipedia. An example edge in the DBpedia knowledge graph is \kbtrip{Larry McCray}{genre}{Blues}, meaning Larry McCray is a blues musician.
This relationship is expressed through the DBpedia \kbrel{genre} relation, a sub-relation of the high level relation \kbrel{isClassifiedBy}. 
The relation prediction task is to predict the relations (if any) between two nodes in the knowledge graph from the entire set of textual evidence, rather than each sentence separately as in mention level relation extraction. %For example, \kbent{Caribou Coffee} and \kbent{Minnesota} are connected by the \kbrel{location} relation, a fact strongly indicated by the contexts in which they co-occur: 
% \begin{itemize}
% \setlength\itemsep{0.0em}
% \item 
%"On both sides of the entrance were Caribou Coffee shops, the Minnesota version of Starbucks"%, and 
% \item 
%"Plenty of other Minnesota-based brands, ranging from 3M to Caribou Coffee, attempted to pay tribute to Prince, a Minneapolis native".
% \end{itemize} 

% hdfs dfs -cat /common-crawl/dbp/binary/relexMentions.tsv/part-00917 | awk  -F $'\t' '$7!=""' | grep odp | less
%dbr:Salmon_Falls_Creek  dbr:Idaho       dbo:Stream      dbo:Region      [130,148)       [236,241)       >dbo:state,>odp:hasLocation,>dbo:city,>odp:hasLocation  A post shared by Kendra Hien (@kndra3) on Aug 9, 2016 at 8:45pm PDT Bell Rapids Sportsman\u2019s Access Subscribe to 98.3 The Snake on Salmon Falls Creek Reservoir \u2013 Grey\u2019s Landing Bruneau Canyon Overlook \u2013 Bruneau, ID Found a little gem in Idaho.      http://983thesnake.com/free-campsites-close-to-twin-falls/

%dbr:James_Meade dbr:Tony_Atkinson       dbo:Person      dbo:Person      [38,49) [108,121)       <dbo:influencedBy,<odp:sameSettingAs    First I would like to pay  tribute to James Meade and this long tradition of British economists,  including Tony Atkinson, with whom we have been working with a lot and  who is largely the godfather of historical studies of income and wealth.      http://accidentaldeliberations.blogspot.co.uk/2014_11_30_archive.html

%dbr:Civil_Music dbr:Om_Unit     unk     dbo:Artist      [205,216)       [173,180)       <dbo:recordLabel,<odp:coparticipatesWith	skip to main | skip to sidebar Om Unit: Aeolian EP [Video] With the Aeolian EP out now digitally, we have been splashed with not one but two fresh new visuals in support of Om Unit 's brilliant release on Civil Music .      http://92bpm.com/2012/07/om-unit-aeolian-ep-video.html
%dbr:Civil_Music dbr:Om_Unit     unk     dbo:Artist      [90,101)        [0,7)   <dbo:recordLabel,<odp:coparticipatesWith        Om Unit - Dark Sunrise (Feat Tamara Blessa) You can scoop the Aeolian EP now, over at the Civil Music and all proper outlets.   http://92bpm.com/2012/07/om-unit-aeolian-ep-video.html
%dbr:Civil_Music dbr:Om_Unit     unk     dbo:Artist      [27,38) [10,17) <dbo:recordLabel,<odp:coparticipatesWith        Shouts to Om Unit, and the Civil Music mandem.  http://92bpm.com/2011/11/civil-music-sampler-dwnld.html
%dbr:Civil_Music dbr:Om_Unit     unk     dbo:Artist      [174,185)       [165,172)       <dbo:recordLabel,<odp:coparticipatesWith	Desto\u2019s productions have gained DJ support from the likes of Benji B (BBC Radio 1), DJ Shadow (Mo Wax, Island Records), Blackdown (Keysound), Mark Pritchard (Warp), Om Unit (Civil Music) and Slackk (Boxed) to name but a few.        http://11v.swaeg.net/lineup/


%Creating the input (adapt some text from CC-DBP paper)

%Source train, Target train, validate and test


%key terms:
%  full/source training data
%  target training data
%  source model
%  transfer learned target model M_t_s
%  target model trained without transfer learning


% Notation
% $T = (t_i, ..., t_N)$
% $M$ source tasks $S = (s_j, ..., s_M)$.
% given a target task and dataset $t_i$, a model $M(t_i,s_j)$ is generated by first training on a source task and dataset $s_j$ , and then transferring this information to $t_i$,
% M(t_i, \phi) for no transfer

% could measure improvement ratio or improvement amount

%As is typical in natural language processing and knowledge induction, the architecture is not nearly as deep as the image classification architecture. 
Figure \ref{fig.rkiarch} shows the relation prediction neural architecture. %The architecture is typical of natural language processing and knowledge induction.
The feature representations are taken from the penultimate layer, the max-pooled network-in-network. All models have the same architecture and hyperparameters, shown in Table \ref{tbl.rkihypers}
%relation prediction neural architecture
\begin{figure}[htb]
   \centering
	\begin{minipage}{.70\textwidth}
	\centering
	\includegraphics[width=0.9\linewidth]{figures/knowledgeArchBasic.pdf}
   \caption{Deep Learning Architecture for Relation Prediction}
   \label{fig.rkiarch}
	\end{minipage}%
\begin{minipage}{.3\textwidth}
   \centering
\begin{center}
\captionof{table}{Hyperparameters used}\label{tbl.rkihypers}
\begin{tabular}{rr}
\toprule 
\bf Hyperparameter & \bf Value \\ \midrule
word dim. & 50 \\
position dim. & 5 \\
sentence vector & 400 \\
NiN filters & 400 \\
CNN filters & 1000 \\
CNN filter width & 3 \\
dropout & 0.5  \\
%learnRate & 0.003 \\
%decay multiplier & 0.99 \\ %This is only for training the target models
%batch size & 16 \\
%optimizer & SGD \\
%minLearnRate = 1.0E-4
\bottomrule
\end{tabular}
\end{center}

\end{minipage}
\end{figure}


We split the task of relation prediction into seven subtasks composed of the high-level relations with the most positive examples in the CC-DBP (other relations were discarded). This was intended to be mirror the partitions of ImageNet by high-level class. The seven source domains are shown in Table \ref{tbl.ccdbpSourceBinary}.
A model is trained for each of these domains on the full training data for the relevant relation types.

%Descriptions from:
%http://www.ontologydesignpatterns.org/ont/dul/DUL.owl
\begin{table}[htb]
\centering
\caption{Source domains division of CC-DBP for binary relation extraction}
\label{tbl.ccdbpSourceBinary}
\begin{tabular}{rrr}
\toprule
Division Name & Number of Relations & Positives in Train \\
\midrule
coparticipatesWith & 227 & 78598\\ 
%A relation between two objects participating in a same Event; e.g., 'Vitas and Jimmy are playing tennis'.
hasLocation & 85 & 72065\\ 
% A generic, relative spatial location, holding between any entities. E.g. 'the cat is on the mat', 'Omar is in Samarcanda', 'the wound is close to the femural artery'.
sameSettingAs & 169 & 40359\\ 
%A relation between two entities participating in a same Situation; e.g., 'Our company provides an antivenom service' (the situation is the service, the two entities are the company and the antivenom).
isClassifiedBy & 34 & 22743\\ 
%A relation between a Concept and an Entity, e.g. 'John is considered a typical rude man'; your last concert constitutes the achievement of a lifetime; '20-year-old means she's mature enough'.
hasPart & 64 & 12319\\ 
%A schematic relation between any entities, e.g. 'the human body has a brain as part', '20th century contains year 1923', 'World War II includes the Pearl Harbour event'. Subproperties and restrictions can be used to specialize hasPart for objects, events, etc.
hasMember & 45 & 36706\\ 
%A relation between collections and entities, e.g. 'my collection of saxophones includes an old Adolphe Sax original alto' (i.e. my collection has member an Adolphe Sax alto).
hasRole & 4 & 7320\\ 
%A relation between an object and a role, e.g. the person 'John' has role 'student'.
\bottomrule
\end{tabular}
\end{table}


% explain it layer by layer
%\begin{enumerate}
%\item Word vectors are pre-trained by word2vec~\cite{word2vec}
%\item Position embeddings encode the distance of each word to each argument.
%\item CNN is applied over each sentence representation
%\item Piecewise max-pooling max-pools the CNN output for each segment of the sentence: before the first argument, between the arguments and after the last argument \cite{zeng2015distant}
%\item A fully connected layer produces the final sentence vector representation
%\item Network-in-network~\cite{lin2013nin} aggregates over the sentence vectors using width-1 CNN
%\item Simple max-pool gathers the aggregation to a fixed length vector
%\item Vector representation for a context set used for vector averaging and distance between domain computations
%\item Fully connected layer transforms the context set representation into predictions for each relation
%\item Relation predictions give the probability for each relation
%\end{enumerate}





